BreakBot: Analyzing the Impact of Breaking Changes to Assist Library Evolution

"If we make this change to our code, how will it impact our clients?" It is difficult for library maintainers to answer this simple-yet essential!-question when evolving their libraries. Library maintainers are constantly balancing between two opposing positions: make changes at the risk of breaking some of their clients, or avoid changes and maintain compatibility at the cost of immobility and growing technical debt. We argue that the lack of objective usage data and tool support leaves maintainers with their own subjective perception of their community to make these decisions. We introduce BreakBot, a bot that analyses the pull requests of Java libraries on GitHub to identify the breaking changes they introduce and their impact on client projects. Through static analysis of libraries and clients, it extracts and summarizes objective data that enrich the code review process by providing maintainers with the appropriate information to decide whether-and how-changes should be accepted, directly in the pull requests.

==> evaluation.tex <==
\section{``Evaluation''}

\begin{itemize}
	\item I changed my mind regarding the evaluation:
	\begin{enumerate}
		\item There are actually many NIER papers without any sort of evaluation
		\item What would a Pilot Study or Accuracy Analysis bring? It would evaluate the tool, BreakBot. But BB isn't ready (reports, all BCs, performance, \etc), and our prototype implementation is \emph{one} instantiation of \emph{zero} policy for \emph{one} language. It doesn't make sense to evaluate it here:~first, we need to discuss the values/policies/practices of one ecosystem/library, then tune the tool for it, then gather users' opinions.
		\item Instead, we should double down on the \emph{vision} of assisting maintainers in evolving their APIs, regardless of particular ecosystems, tools, and languages.
		\item BB is still a central part of the paper as it exemplifies what he could look like (so, screenshots ;)!). But its evaluation shall be done in later papers.
	\end{enumerate}
\end{itemize}

\paragraph{BreakBot's accuracy}
Do we accurately detect BCs? Do we accurately assess their impact? \etc.

\paragraph{Pilot Study: the Spoon library}
Is the tool providing useful information? What are the pain points and things to improve?

